AI-aided Geometric Design of Anti-infection Catheters

Bacteria can swim upstream due to hydrodynamic interactions with the fluid flow in a narrow tube, and pose a clinical threat of urinary tract infection to patients implanted with catheters. Coatings and structured surfaces have been proposed as a way to suppress bacterial contamination in catheters. However, there is no surface structuring or coating approach to date that thoroughly addresses the contamination problem. Here, based on the physical mechanism of upstream swimming, we propose a novel geometric design, optimized by an AI model predicting in-flow bacterial dynamics. The AI method, based on Fourier neural operator, offers significant speedups over traditional simulation methods. Using Escherichia coli, we demonstrate the anti-infection mechanism in quasi-2D micro-fluidic experiments and evaluate the effectiveness of the design in 3Dprinted prototype catheters under clinical flow rates. Our catheter design shows 1-2 orders of magnitude improved suppression of bacterial contamination at the upstream end of the catheter, potentially prolonging the in-dwelling time for catheter use and reducing the overall risk of catheter-associated urinary tract infections.

==> sections/4-discussion.tex <==
\section*{Discussion}\label{sec12}

In this work, we introduce an effective geometrical design principle for suppressing bacterial upstream swimming and super-contamination. The design is relatively simple to manufacture and does not require additional steps to the regular clinical protocols, or retraining of medical personnel. We note that the geometrical design cannot completely eliminate bacterial upstream swimming, especially at near-zero flow rates. However, it drastically reduces the amount of super-contamination and may significantly prolong the indwelling time of catheters. Moreover, our solution does not introduce chemicals into the catheters, and thus is safe and does not require additional maintenance. In addition, our geometrical design approach has excellent compatibility with other procedural measures, anti-bacterial surface modification, and environmental control methods. 

==> sections/S1-supplements.tex <==
% \bmhead{Supplementary information}

% If your article has accompanying supplementary file/s please state so here. 

% Authors reporting data from electrophoretic gels and blots should supply the full unprocessed scans for key as part of their Supplementary information. This may be requested by the editorial team/s if it is missing.

% Please refer to Journal-level guidance for any specific requirements.
